On the Scalability of Reliable Data Transfer in High Speed Networks

This paper considers reliable data transfer in a high-speed network (HSN) in which the per-connection capacity is very large. We focus on sliding window protocols employing selective repeat for reliable data transfer and study two reliability mechanisms based on ARQ and FEC. The question we ask is which mechanism is more suitable for an HSN in which the scalability of reliable data transfer in terms of receiver's buffer requirement and achievable delay and throughput is a concern. To efficiently utilize the large bandwidth available to a connection in an HSN, sliding window protocols require a large transmission window. In this regime of large transmission windows, we show that while both mechanisms achieve the same asymptotic throughput in the presence of packet losses, their delay and buffer requirements are different. Specifically, an FEC-based mechanism has delay and receiver's buffer requirement that are asymptotically smaller than that of an ARQ-based selective repeat mechanism by a factor of log W, where W is the window size of the selective repeat mechanism. This result is then used to investigate the implications of each reliability mechanism on protocol design in an HSN in terms of throughput, delay, buffer requirement, and control overhead.

==> model.tex <==

\section{System Model} \label{s:model}

